Constant factor FPT approximation for capacitated k-median

Capacitated k-median is one of the few outstanding optimization problems for which the existence of a polynomial time constant factor approximation algorithm remains an open problem. In a series of recent papers algorithms producing solutions violating either the number of facilities or the capacity by a multiplicative factor were obtained. However, to produce solutions without violations appears to be hard and potentially requires different algorithmic techniques. Notably, if parameterized by the number of facilities $k$, the problem is also $W[2]$ hard, making the existence of an exact FPT algorithm unlikely. In this work we provide an FPT-time constant factor approximation algorithm preserving both cardinality and capacity of the facilities. The algorithm runs in time $2^{\mathcal{O}(k\log k)}n^{\mathcal{O}(1)}$ and achieves an approximation ratio of $7+\varepsilon$.

==> fptback.tex <==
\section{FPT Algorithm}

\begin{definition}
An instance of \CKM is called $\ell$-\emph{centered} if the metric $d$ over $F \cup C$ is induced by a weighted graph $G(V,E)$ with a subset $W \subseteq V,\, |W|\le \ell$, such that for $uv \in E$ either $u$ or $v$ belongs to $W$.
\end{definition}

Consider an (uncapacitated) assignment $\psi : C \to S$ of clients to $\ell$ open facilities, such that each client is connected to the closest open facility.†
We can use $\psi$ to transform an arbitrary instance of CKM to an $\ell$-centered instance.
We maintain the metric $d$ over the set of open facilities and each other point in $F \cup C$ is connected by an edge to the closest open facility.
Let us denote the new metric as $d^\psi$.

\begin{lem}\label{lem:metric-switch}
Let $cost(\phi, d) = \sum_{c \in C}d(c, \phi(c))$.
For any mappings $\phi, \psi : C \to S$ it holds
\begin{equation*}
cost(\phi, d) \le cost(\phi, d^\psi) \le 3\cdot cost(\phi, d) + 4\cdot cost(\psi, d).
\end{equation*}
\end{lem}

\begin{lem}\label{lem:fpt-uniform}
\UCKM can be solved exactly in time $\ell^kn^{O(1)}$ on $\ell$-centered instances. 
\end{lem}

\begin{lem}\label{lem:fpt-non-uniform}
\NUCKM can be solved with approximation ratio $(1+\epsilon)$ in time $(\ell + k/ \epsilon)^{O(k)} n^{O(1)}$ on $\ell$-centered instances. 
\end{lem}

\begin{thm}
\NUCKM can be solved with approximation ratio $(7+\epsilon)$ in time $(k/ \epsilon)^{O(k)}n^{O(1)}$.
\end{thm}
\begin{proof}
We begin with relaxing the problem to the uncapacitated version and then we use rounding procedure by [TODO] to open at most $\ell = (1+\frac 1 \epsilon)\cdot k \cdot \ln n$ facilities while exceeding the optimal cost by factor $1+\epsilon$.
Therefore we have obtained a mapping $\psi$, such that $cost(\psi,d) \le (1+\epsilon)\cdot Opt$ and $(F,C,d^\psi)$ is an $\ell$-centered instance.

Lemma~\ref{lem:metric-switch} guarantees that the cost of the optimal solution in instance $(F,C,d^\psi)$ is at most $(7+4\eps)\cdot Opt$.
Now we can find an assignment being a $(1+\epsilon)$-approximation with Lemma~\ref{lem:fpt-non-uniform}.
Its cost after returning to the original instance $(F,C,d)$ cannot increase.
The claim follows.
\end{proof}

\section{Lower bound}

In this section we argue that allowing factor $f(k)$ in the running time for $k$-median should not help in finding an exact solution and we still need to settle for approximation.

\begin{thm}
The $k$-median problem is \WW-hard when parameterized by $k$, even on unweighted graphs.
\end{thm}
\begin{proof}
Easy reduction from \textsc{Dominating Set}. 
\end{proof}


==> preliminaries.tex <==
% !TEX root = main.tex

\section{Preliminaries}\label{sec:preliminaries}
\micr{these are not only preliminaries but related work as well. some reorganization?}
    In the \textsc{Capacitated \(k\)-Median} problem (\CKM{}), we are given a
    set \(F\) of facilities, each facility \(f\) with a capacity \(u_f \in
    \mathbb{Z}_{\geqslant 0}\), a set \(C\) of clients, a  metric \(d\) over \(F
    \cup C\) and an upper bound \(k\) on the number of facilities we can open.
    A solution to the \CKM problem is a set \(S \subseteq F\) of at most \(k\) open facilities
    and a connection assignment \(\phi: C \to S\) of clients to open facilities
    such that \(\size{\phi^{-1}(f)} \leqslant u_f\) for every facility \(f \in S\).
    The goal of the problem is to find a solution that minimizes the connection cost \(\sum_{c \in C}d(c, \phi(c))\).

    \paragraph{Uncapacitated \(k\)-median} The standard \(k\)-median problem,
    where there is no restriction on the number of clients served by a facility,
    can be approximated up to a constant factor~\cite{charikar1999constant,
    arya2004local}. The current best is the \((2.675+\epsilon)\)-approximation
    algorithm of Byrka et al.~\cite{byrka2015improved}, which is a result of
    optimizing a part of the algorithm of Li and
    Svensson~\cite{li2013approximating}.

    \paragraph{Approximability of \CKM{}} Capacitated \(k\)-median is among the
    few remaining fundamental optimization problems for which it is not clear if
    there exist polynomial time constant factor approximation algorithms. All
    the known algorithms violate either the number of facilities or the
    capacities. In particular, already the algorithm of Charikar et
    al.~\cite{charikar1999constant} gave 16-approximate solution for uniform
    capacitated \(k\)-median violating the capacities by a factor of 3. Then
    Chuzhoy and Rabani~\cite{chuzhoy2005approximating} considered general
    capacities and gave a 50-approximation algorithm violating capacities by a
    factor of 40.

    The difficulty appears to be related to the unbounded integrality gap of the
    standard LP relaxation. To obtain integral solutions that are bounded with respect to
    a fractional solution to the standard LP, one has to either allow the
    integral solution to open twice as much facilities or to violate the capacities
    by a factor of two. LP-rounding algorithms essentially matching these limits
    were obtained~\cite{aardal2015approximation, BFRS15}.

    Subsequently,  Li  broke  this  integrality  gap  barrier  by  giving  a
    constant  factor  algorithm  for  capacitated k-median by opening \((1 +
    \eps) \cdot k\) facilities~\cite{Li15uniform,Li16non_uniform}. Then
    analogous results, but violating the capacities by a factor of \((1 +
    \eps)\) were also
    obtained~\cite{DBLP:conf/ipco/ByrkaRU16,DBLP:conf/icalp/DemirciL16}.

    The algorithms with \((1+\eps)\) violations are all based on strong LP
    relaxations containing additional constraints for subsets of facilities.
    Notably, it is not clear if these relaxations can be solved exactly in
    polynomial time, still they suffice to construct an approximation algorithm
    via a ``round-or-separate” technique that iteratively adds consistency
    constraints for selected subsets. Although while spectacularly breaking the
    standard LP integrality bound, these techniques appear insufficient to yield
    a proper approximation algorithm that does not violate constraints.

\mar{
The only true approximation for \CKM{} known is a folklore \(\OO\br{\log k}\) approximation algorithm
    that can be obtained via metric tree embedding with expected logarithmic
    distortion~\cite{FakcharoenpholRT03}.}
\mic{To the best of our knowledge,
this result has not been explicitly published, but it can be obtained similarly to the \(\OO\br{\log k}\)-approximation for \UKM by Charikar~\cite{DBLP:conf/stoc/CharikarCGG98}.
For the sake of completeness and since it follows easily from our framework, we give its proof in Section~\ref{sec:folklore} without claiming credit for it. } \marr{Previously it was written that the $\lg k$-approximation was indicated in the work of~\cite{charikar1999constant} but after looking at this paper I don't think it's the case}

    This \(\OO\br{\log k}\)-approximation is in contrast with other
    capacitated clustering problems such as facility location and k-center,
    for which constant factor approximation algorithms are
    known~\cite{korupolu2000analysis,cygan2012lp}.


%The uncapacitated $k$-median problem is very much the same as \CKM defined above  except that we do not have upperbounds $u_f$ for facilities, and so each facility can serve as many clients as we shall connect to it.

    \paragraph{\textsc{Uniform CKM}} In the case when all the facilities can
    serve at most \(u\) clients, for some integer \(u\), we get the
    \textsc{Uniform \CKM} problem. \mar{Although our \((7+\eps)\)-approximation for the non-uniform case yields a result for this version as well, we present a derivation for this case separately as it allows for a gradual presentation of our ideas.}

    \paragraph{Parameterized Complexity} A parameterized problem instance is
    created by associating an input instance with an integer parameter \(k\). We
    say that a problem is \emph{fixed parameter tractable} (\FPT{}) if any
    instance \((I, k)\) of the problem can be solved in time
    \(f(k)\cdot |I|^{\OO(1)}\), where \(f\) is an arbitrary computable function of
    \(k\). Throughout this paper, we use the standard notation \(\OO^*\) to hide
    factors polynomial in \(|I|\).\footnote{That is,
    \(\OO^*(f(k))=f(k)\cdot|I|^{\OO(1)}\).} We say that a problem is \FPT{} if
    it is possible to give an algorithm solving it with running time of the
    required form, called as a \emph{parameterized algorithm}.

    To show that a
    problem is unlikely to be \FPT{}, we use parameterized reductions analogous
    to those employed in Classical Complexity. Here, the concept of
    \textsf{W}-hardness replaces the one of \NP-hardness, and we need not only
    construct an equivalent instance in \FPT{} time, but also ensure that the
    size of the parameter in the new instance depends only on the size of the
    parameter in the original instance.
\mic{In contrast to the \NP-hardness theory, there is a hierarchy of classes $\FPT = \textsf{W[0]} \subseteq \textsf{W[1]} \subseteq \textsf{W[2]} \subseteq \dots$ and these containments are believed to be strict.
If there exists a parameterized reduction transforming a problem known to
    be \textsf{W[t]}-hard for $t>0$ to another problem \(\Pi \), then the problem \(\Pi \) is
    \textsf{W[t]}-hard as well. This implies that \(\Pi \) does not admit an algorithm with
    running time \(\OO^*(f(k))\) unless the \textsf{W}-hierarchy collapses.}

\paragraph{} We begin with an argument that allowing \FPT time  for (even uncapacitated) \textsc{$k$-Median} should not help in finding the optimal solution and we still need to settle for approximation.

\begin{fact}
The \textsc{Uncapacitated $k$-Median} problem is \WW-hard when parameterized by $k$, even on metrics given by unweighted graphs.
\end{fact}
\begin{proof}
Consider an instance of the \textsc{Dominating Set} problem,
which is \WW-hard when parameterized by the solution size.
A dominating set of size at most $k$ exists in graph $G$ if and only if we can find a vertex set $S$ of size $k$, such that all other vertices are at distance 1 from $S$.
This is equivalent to the solution to \textsc{Uncapacitated $k$-Median} on the metric induced by $G$ being exactly $|V(G)|-k$. \mesr{Is the cost function a metric in the reduction ?}
\end{proof}

\paragraph{Parameterized Approximations}
In recent years new research directions emerged in the intersection of the theory of approximation algorithms and the \FPT{} theory.
It turned out that for some problems that are either \W-hard \micr{TODO} parameterization still comes in useful when we want to reduce the approximation ratio.
Some examples are $(2-\eps)$-approximation for \textsc{$k$-Cut}~\cite{gupta2018fpt} or
$\OO(\log k)$-approximations for \textsc{$k$-Vertex Separator}\cite{Lee18} and \textsc{$k$-Treewidth Deletion}~\cite{gupta-arxiv}.\micr{anything more?}

On the other hand some problems have been proven resistant to such improvements.
Chalermsook et al.~\cite{pasin-focs17} observed the under the assumption of $\textsf{Gap-ETH}$ there can be no parametrized approximation with ratio $o(k)$ for \textsc{$k$-Clique} and none with ratio
$f(k)$ for \textsc{$k$-Dominating Set} (for any function $f$).
Subsequently $\textsf{Gap-ETH}$ has been replaced with a better established hardness assumption $\FPT \ne \W$ for \textsc{$k$-Dominating Set}~\cite{pasin-stoc18}.

\iffalse
\paragraph{} Relying on this result, we can rule out the existence of an exact \FPT time for (even uncapacitated) \textsc{$k$-Median}.
What is more, it does help if my relax the problem and look for solution that open at most $f(k)$ facilities for any function $f$.
This means that from the perspective of parameterized complexity
we still need to settle for approximation.
\fi
